Optimizing Distributed Training on Frontier for Large Language Models

Large language models (LLMs) have demonstrated remarkable success as foundational models, benefiting various downstream applications through fine-tuning. Recent studies on loss scaling have demonstrated the superior performance of larger LLMs compared to their smaller counterparts. Nevertheless, training LLMs with billions of parameters poses significant challenges and requires considerable computational resources. For example, training a one trillion parameter GPT-style model on 20 trillion tokens requires a staggering 120 million exaflops of computation. This research explores efficient distributed training strategies to extract this computation from Frontier, the world's first exascale supercomputer dedicated to open science. We enable and investigate various model and data parallel training techniques, such as tensor parallelism, pipeline parallelism, and sharded data parallelism, to facilitate training a trillion-parameter model on Frontier. We empirically assess these techniques and their associated parameters to determine their impact on memory footprint, communication latency, and GPU's computational efficiency. We analyze the complex interplay among these techniques and find a strategy to combine them to achieve high throughput through hyperparameter tuning. We have identified efficient strategies for training large LLMs of varying sizes through empirical analysis and hyperparameter tuning. For 22 Billion, 175 Billion, and 1 Trillion parameters, we achieved GPU throughputs of $38.38\%$, $36.14\%$, and $31.96\%$, respectively. For the training of the 175 Billion parameter model and the 1 Trillion parameter model, we achieved $100\%$ weak scaling efficiency on 1024 and 3072 MI250X GPUs, respectively. We also achieved strong scaling efficiencies of $89\%$ and $87\%$ for these two models.

==> counting-flops.tex <==
\section{Counting FLOPS}

\subsection{Counting Hardware FLOPS}
We collect the following hardware counters to count the total FLOPS.

\begin{verbatim}
       'SQ_INSTS_VALU_ADD_F16',
       'SQ_INSTS_VALU_MUL_F16', 'SQ_INSTS_VALU_FMA_F16',
       'SQ_INSTS_VALU_TRANS_F16', 'SQ_INSTS_VALU_MFMA_MOPS_F16',
       'SQ_INSTS_VALU_ADD_F32', 'SQ_INSTS_VALU_MUL_F32',
       'SQ_INSTS_VALU_FMA_F32', 'SQ_INSTS_VALU_TRANS_F32',
       'SQ_INSTS_VALU_MFMA_MOPS_F32', 'SQ_INSTS_VALU_ADD_F64',
       'SQ_INSTS_VALU_MUL_F64', 'SQ_INSTS_VALU_FMA_F64',
       'SQ_INSTS_VALU_TRANS_F64', 'SQ_INSTS_VALU_MFMA_MOPS_F64',
       'SQ_INSTS_VALU_MFMA_BF16', 'SQ_INSTS_VALU_MFMA_MOPS_BF16'
\end{verbatim}


Then, we use the following formula to calculate the total FLOPS.

\begin{verbatim}
    
flops_fp16 = 64 * (SQ_INSTS_VALU_MUL_F16 +
                   SQ_INSTS_VALU_ADD_F16 +
                   2 * SQ_INSTS_VALU_FMA_F16 +
                   SQ_INSTS_VALU_TRANS_F16)

       

flops_mfma = 512 * SQ_INSTS_VALU_MFMA_MOPS_F16 +
512 * SQ_INSTS_VALU_MFMA_MOPS_BF16 +
512 * SQ_INSTS_VALU_MFMA_MOPS_F32 +
512 * SQ_INSTS_VALU_MFMA_MOPS_F64

flops_fp32 = 64 * SQ_INSTS_VALU_MUL_F32 +
                           SQ_INSTS_VALU_ADD_F32 +
                           2 * SQ_INSTS_VALU_FMA_F32 +
                           SQ_INSTS_VALU_TRANS_F32
                           )
flops_fp64 = 64 * (SQ_INSTS_VALU_MUL_F64 +
                           SQ_INSTS_VALU_ADD_F64 +
                           2 * SQ_INSTS_VALU_FMA_F64 +
                           SQ_INSTS_VALU_TRANS_F64
                           )

mixed_flops = flops_mfma + flops_fp16 + flops_fp32 + flops_fp64

\end{verbatim}

\textcolor{red}{Note, in Frontier user guide, the term $flops\_mfma$ has different coefficients (1024, 1024, 256, and 256). But our experiments with simple GEMM operation and discussion with a couple of AMD personnel reveal that values of all these four coefficients is more likely to be 512.}

\subsection{Model Flops}
Megatron-DeepSpeed codebase reports Model FLOPS in the log using a throughput calculator function in megatron/utils.py. We average the FLOPS across iterations to get a final Model FLOPS.

\begin{lstlisting}[language=Python]
    def throughput_calculator(model, args, iteration_time, total_iterations):
        batch_size = args.micro_batch_size * get_num_microbatches() * args.data_parallel_size
    
        approx_parameters_in_billions = None if (model is None) else get_parameters_in_billions(model)
        elapsed_time_per_iter = iteration_time/total_iterations
        samples_per_second = batch_size / elapsed_time_per_iter

        #flops calculator
        hidden_size = args.hidden_size
        num_layers = args.num_layers
        vocab_size = args.padded_vocab_size

        # General TFLOPs formula (borrowed from Equation 3 in Section 5.1 of
        # https://arxiv.org/pdf/2104.04473.pdf).
        # The factor of 4 is when used with activation check-pointing,
        # otherwise it will be 3.
        checkpoint_activations_factor = 3
        if hasattr(args, 'checkpoint_activations') and args.checkpoint_activations:
            checkpoint_activations_factor = 4
        if hasattr(args, 'recompute_granularity') and (args.recompute_granularity == 'selective' or args.recompute_granularity == 'full'):
            checkpoint_activations_factor = 4
        seq_len = args.seq_length
        if hasattr(args, 'actual_seq_length'):
            seq_len = args.actual_seq_length
        flops_per_iteration = (24 * checkpoint_activations_factor * batch_size * seq_len * num_layers * (hidden_size**2)) * (1. + (seq_len / (6. * hidden_size)) + (vocab_size / (16. * num_layers * hidden_size)))
        tflops = flops_per_iteration / (elapsed_time_per_iter * args.world_size * (10**12))
        return samples_per_second, tflops, approx_parameters_in_billions
\end{lstlisting}

We grep TFLOPs in the run log to create the time file which looks like this (Figure~\ref{fig:time-log}).

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{images/times-log.png}
    \caption{Sample time log for model flops computation}
    \label{fig:time-log}
\end{figure}

We calculate the model FLOPS (per GCD, per second) using the formula:

\begin{equation}
    model\_flops = \frac{\sum iteration\ time \times iteration\ FLOPS}{\sum iteration\ time}
\end{equation}


\subsection{Agreement between Hardware FLOPS and Model FLOPS}

These two measures agree very closely. However, there were incidents of disagreement and we have identified erroneous configurations when that happens. There are two ways to define the micro\_batch\_size for training. One in the deepspeed config file through the key $train\_micro\_batch\_size\_per\_gpu$ and another is through the megatron launch parameter $micro\_batch\_size$. These two values need to be the same for correct FLOPS reporting. The latter is used for actual training, and the former is used for FLOPS calculation. If there is a mismatch between these two, the model FLOPS reported gets $\frac{train\_micro\_batch\_size\_per\_gpu}{micro\_batch\_size}$-times of Hardware FLOPS. So, we have to make sure these two parameters are in agreement.

We came to this conclusion from the following experiment (Figure~\ref{fig:flops-experiments}).

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/flops-experiments}
    \caption{Two micro-batch-size parameter needs to be in agreement, otherwise Model FLOPS get mis-reported.}
    \label{fig:flops-experiments}
\end{figure}

==> materials/3D-parallelism-on-Frontier.tex <==
\section{Enabling 3D parallelism on Frontier}
\begin{enumerate}
    \item 3D Parallelism and known trade-offs
    \item Frontier architecture
    \item Porting Megatron-DeepSpeed to Frontier
\end{enumerate}

==> materials/baseline.tex <==
\section{Baseline performance of Frontier GPUs}
\begin{enumerate}
    \item Training a 1.4B model on MI250X GPU
    \item Considerations to improve the throughput
    \item Advantage of FlashAttention
\end{enumerate}

==> materials/batch-size.tex <==
\subsection{Batch-size Used by Other Large Model Training Effort}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline 
        Model Name & \#GPUs & Global Batch-size & Platform & Replica Size\\ \hline 
        Turing-NLG 530B & 3360 & 1920 & Celene, A100, 8x35xZ1 & 280\\ \hline  
        OPT-175B & 992 & 1024 & A100, FSDP X TP(=?) & ? \\ \hline 
        BigScience Bloom 176B & 384 &  2048 & A100, TP=4, PP=12, DP=8, MBS=2 & 48 \\ \hline 
    \end{tabular}
    \caption{Other Large Model Training Setup and Their Max Batch-Size}
    \label{tab:my_label}
\end{table}

==> materials/flops-counting.tex <==
\section{Counting FLOPs}

\begin{enumerate}
    \item Elapsed time: checked, not it
    \item Value overflow?
    \item Overcounting model replicas?
    \item Model parameter count?
    \item Skipped iteration?
    \item ZeRO-1 doing something crazy?
\end{enumerate}

\subsection{Trying rocprof across multiple GPUs}

It works on a single GPU. It works across multiple GPUs too, but not with \begin{verbatim}
    --timestamp on:wq
    
\end{verbatim}

\subsection{Collecting Harware Counters}

\paragraph{Collect Total Flops: Collect Counters for Every Kernel Calls without time information}

\begin{verbatim}
    rocprof -i inputs-fp16.txt -o profs3.6b-notrain/${outfile} python pretrain_gpt.py
\end{verbatim}

The output table looks like:

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/header.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/body.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\subsection{Collect Total Duration for the Kernel Launches During Training}

We first run the training with same configuration without the rocprof and measure the total time ($t_{total}$). Then, we comment out the training loop, and rerun the code without rocprof. The elapsed time for the secod run is $t_{overhead}$. We get a ceiling of the actual training time $t_{training} = t_{total} - t_{overhead}$.

\subsection{Collect FLOPS During Overhead}
With the commented out training loop, we again run the code with rocprof to find out the kernel calls unrelated to the training loop.

\begin{verbatim}
    rocprof -i inputs-fp16.txt -o profs3.6b-notrain/${outfile} python pretrain_gpt_notrain.py
\end{verbatim}


\subsection{Hardware FLOPs}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    \hline
       Model  & Hardware TFLOPs & Model TFLOPs & DP Size \\ \hline  
         87B & - & 216 & 2 \\ \hline 
         22B & 133 & 205 & 2 \\ \hline 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline
    FlashAttention & Model TFLOPS & HW TFLOPS & Model TFLOPs/GCD & HW TFLOPs/GCD \\ \hline 
         Not used &  146836.96 & 72523.64 & 140.18 &  69.24\\ \hline 

    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}



==> materials/growing-175b.tex <==
\subsection{Growing 175B model to larger models}
\begin{enumerate}
    \item GPT architecture and model-size
    \item Growing depth
    \item Growing width
\end{enumerate}

==> materials/results.tex <==
\section{Results}

\subsection{Achieved Throughput Using Hardware Counters for Three Models}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/MI250X-Throughput.pdf}
    \caption{MI250X Throughput for various model sizes}
    \label{fig:mi250x-throughput}
\end{figure}

\subsection{Throughput as a Function of Global Batch Size}
\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/tflops-vs-gbs-22b.pdf}
    \caption{Throughput vs global batch-size for 22B model.}
    \label{fig:tflops-vs-gbs-22b}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/tflops-vs-gbs-1T.pdf}
    \caption{Throughput vs global batch-size for 1T model.}
    \label{fig:tflops-vs-gbs-1T}
\end{figure}




==> materials/techniques.tex <==
\subsection{Lessons Learned}%Optimal Training Techniques}

\subsubsection{\textit{bf16} Precision}
There are four precision considerations for training a large language model, fp16, bf16, fp32, and mixed-precision. While using fp16 and bf16, parameters, optimizers, and gradients are saved using 16-bit data-type. In fp32 precision, these values are saved in 32-bit parameters. In mixed-precision training, 

\paragraph{ChatGPT Answer}

{\color{blue} BF16, FP16, and FP32 are different data formats used for representing real numbers in computing. FP32 (Single Precision) is a 32-bit format with a wide range and high precision, suitable for most general applications. FP16 (Half Precision) is a 16-bit format that sacrifices precision for reduced storage and computational requirements, making it popular in resource-constrained environments like mobile devices and some GPUs. BF16 (Bfloat16) is a 16-bit format designed to balance the precision of FP32 and the efficiency of FP16. BF16 is often used in deep learning and AI applications, offering better stability during training and improved model accuracy compared to FP16 while still providing some resource advantages. The choice of format depends on the specific application's requirements and the trade-offs between precision and efficiency.}
\begin{comment}
What's the difference between bf16, fp16, and fp32?
 ChatGPT
BF16 (Bfloat16), FP16 (Half Precision), and FP32 (Single Precision) are different data formats used in computing and represent various levels of precision for representing real numbers. In mixed precision training, both fp16 and fp32 data-types are used. BF16 provides the best of fp16 and fp32 by requiring less memory and providing higher precision.

FP32 (Single Precision):

FP32 is a 32-bit floating-point format that is commonly used in most computer systems.
It consists of 1 sign bit, 8 exponent bits, and 23 significand (mantissa) bits.
FP32 provides a wide range of values and a relatively high level of precision, making it suitable for many general-purpose applications.
It is commonly used in scientific computing, graphics, and machine learning.
FP16 (Half Precision):

FP16 is a 16-bit floating-point format.
It consists of 1 sign bit, 5 exponent bits, and 10 significand bits.
FP16 sacrifices precision in exchange for reduced storage and computational requirements.
It is commonly used in applications where memory and computational resources are limited, such as mobile devices, some GPUs, and deep learning accelerators.
While FP16 can represent a wide range of values, it has limited precision, and numerical instability can occur in some calculations.
BF16 (Bfloat16):

BF16 is a 16-bit "brain floating-point" format designed to strike a balance between the storage efficiency of FP16 and the precision of FP32.
It consists of 1 sign bit, 8 exponent bits, and 7 significand bits.
BF16 is particularly popular in the context of deep learning and artificial intelligence, where it can be used for neural network training and inference.
Its greater significand precision compared to FP16 allows for more stable training and improved model accuracy compared to straight FP16, while still offering some of the memory and computational advantages of 16-bit formats.
In summary, the key differences among these formats are the number of bits allocated to the exponent and significand, which determine the range and precision of numbers that can be represented. Choosing the right format depends on the specific application and trade-offs between precision and resource efficiency.
\end{comment}

\subsubsection{RCCL Plugin by AWS}
\textcolor{red}{[PARAPHRASE] AWS OFI RCCL is a plug-in which enables EC2 developers to use libfabric as a network provider while running AMD's RCCL based applications.}. On Frontier, usage of this plugin shows performance improvement of up to $10\%$.

\subsubsection{Pipeline Saturation by increasing number of micro-batches}
We use pipeline parallelism provided by DeepSpeed (from DeepSpeed-Megatron, but not the Megatron's version). This pipeline parallelism algorithm is PipeDream's algorithm where multiple stages are overlapped and 1F1B algorithm is followed to reduce the bubble size. However, if the pipeline stages are not saturated, the bubble size will increase. To ensure the saturation, the number of micro-batches must be equal to or more than the number of pipeline stages.

\subsubsection{Activation Checkpointing to Increase Per GPU Batch-size}
To achieve high per-GPU compute utilization, we need to facilitate large micro-batch size. However, large batch creates large activation memory requirement and the program runs into OOM error. To overcome this, we deploy activation checkpointing, which at the cost of 30\% extra computation provides much higher compute utilization.

\subsection{Limiting Tensor-Parallelism to A Single GPU}
Since the AllReduce operation is too frequent and needs to be performed for every layer, a layer spread across nodes cause tree-based AllReduction between GPUs across nodes and the communication latency becomes a significant bottleneck.

\subsubsection{Flash-Attention}
Using Flash-attention improved throughput by $30\%$.

\subsubsection{Using/Not-using ZeRO-1 Optimizer}
Using ZeRO-1 hasn't shown any apparent benefit.

==> materials/training-175b.tex <==
\section{Distributed Training of a 175B model on Frontier}

\subsection{Model Architecture}
We select GPT3 Model's architecture as our 175B model architecture. We listed the specifics in Table~\ref{tab:model-arch}. 

\begin{table}[h]
\centering
\caption{The specification of GPT-style LLMs}\label{tab:model-arch}
\begin{tabular}{ccccc}
\hline
Model & \#layers & Hidden size & \#attention heads & \#Nodes\\ \hline
1.4B  & 24 & 2,064       & 24      &   4 (1)\\ \hline
175B  & 96  & 12,288      & 96      &  12\\ \hline
1T    & 128 & 25,600      & 128     & 128 (64)\\ \hline
\end{tabular}
\end{table}

\subsection{Memory Requirement}
The memory requirement for training such a model is 3.5 TB to 4.2 TB (Table~\ref{tab:mem-175b}. One Frontier MI250X GCD has 64 GB of memory, so it will require 55-65 GCDs, which translates to 7-9 Frontier nodes. 

\begin{table}[h]
    \centering
    \begin{tabular}{c | c c c}
    \hline 
         &  \multicolumn{3}{c}{Memory Requirement}\\ \cline{2-4}
         Values & fp16/bf16 (2B) & fp32 (4B) & Mixed-Precision (6B) \\ \hline \hline 
         Parameters & 350 GB & 750 GB & 1.05 TB \\ \hline 
         Gradients & 1.05 TB & 1.05 TB & 1.05 TB \\ \hline 
         Optimizer States & 2.1 TB & 2.1 TB & 2.1 TB \\ \hline \hline 
         Total Memory & 3.5 TB & 3.9 TB & 4.2 TB \\ \hline 
    \end{tabular}
    \caption{Memory Requirement for Training a 175B Model in different precision. We have not included the activation memory or the overhead memory for various distribution framework.}
    \label{tab:mem-175b}
\end{table}

\subsection{Distribution Strategy}
With 96 Layers and 12,288 hidden-size, there are several considerations for Tensor parallelism and Pipeline parallelism. 

\paragraph{Granularity} First is to ensure that we don't break the model into too small parts so that very little computation can happen before the communication happens and the communication latency takes over the overall training time. We have found that a model size of 1.4B per GCD usually achieves the best performance on MI250X GCDs. We choose 16 nodes, so that the size of the model partition on each GCD is ~1.4B.

\paragraph{Tensor Parallelism} Second consideration is to limit the Tensor parallelism within a node, as Tensor parallelism across the nodes has demonstrated implication of high communication latency. Since a Frontier node has 8 MI250X GCDs, and they are connected pair-wise, the search-space for Tensor parallelism will be $\{1, 2, 4, 8\}$.


\paragraph{Pipeline Parallelism} Third consideration is lowering the volume of communication bubble by not introducing too many pipeline stages. To ensure load-balance, the number of pipeline stages should occupy same number of layers. Hence, the search-space for Pipeline Parallelism is $\{1, 2, 3, 4, 8, 16, 32, 48\}$.

\subsection{Best Strategy to Train a 175B Model}

We rate a distribution strategy based on the achieved per GCD throughput in TFLOPs. The following Table lists the values for each of the distribution parameters. We achieved \textcolor{red}{149.09 TFLOPs} per GCD with this distribution combination.


\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
    \hline 
     Parameter    &  Value \\ \hline \hline 
       TP  & 4 \\ \hline 
       PP & 16 \\ \hline 
       MBS & 1 \\ \hline 
       GBS & 1280 \\ \hline 
       ZeRO Stage & \textcolor{red}{1} \\ \hline 
       Flash Attention & True \\ \hline 
       Precision & fp16 \\ \hline 
       checkpoint-activations & True \\ \hline 
    \end{tabular}
    \caption{Best parameters for training a 175B model}
    \label{tab:best-params-175b}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
    \hline 
     Strategy    & Throughput \\ \hline 
        PP + TP + ZeRO-1 + & 133 TFLOPs \\ \hline 
        PP + TP + ZeRO-1 + FlashAttention & 143.9 TFLOPs \\ \hline 
        PP + TP + ZeRO-1 + FlashAttention + AWS-OFI-RCCL & 149.09 TFLOPs \\ \hline  
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{comment}
    
\subsection{Scaling with Data Parallel Training}
Figure~\ref{fig:strong-scaling-175b} shows that we can achieve 98.6\% strong scaling efficiency when we do a data-parallel training of 175B model by linearly increasing the global batch-size.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{images/strong-scaling-175b-bf16.pdf}
    \caption{Strong scaling with data parallel training of 175B model.}
    \label{fig:strong-scaling-175b}
\end{figure}


\end{comment}




\begin{enumerate}
    \item Identifying the right strategy to distribute using various parallelisms
    \item DeepHyper parameter tuning to find the best strategies
    \item Profiling performance of three different parallelisms, communication patters, throughput
    \item Lessons learned
\end{enumerate}

==> materials/training-1T.tex <==
\section{Training a Trillion Parameter Model}

\paragraph{Best Performance So Far:} \textcolor{red}{48.01 TFLOPs}

\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
    \hline 
     Parameter    &  Value \\ \hline \hline 
       TP  & 4 \\ \hline 
       PP & 128 \\ \hline 
       MBS & 1 \\ \hline 
       GBS & \textcolor{red}{1024*} \\ \hline 
       ZeRO Stage & 0 \\ \hline 
       Flash Attention & True \\ \hline 
       Precision & \textcolor{red}{bf16*} \\ \hline 
       checkpoint-activations & True \\ \hline 
    \end{tabular}
    \caption{Best parameters for training a 1T model}
    \label{tab:best-params-175b}
\end{table}


\begin{enumerate}
    \item Finding the right architecture and amount of resources
    \item Pipeline parallelism: how to saturate the pipeline stages
    \item Tensor parallelism: the limit
    \item ZeRO optimizer -- pros vs cons
    \item Need for Activation checkpointing
    Activation checkpointing frees up memory to make room for the activation and accumulated gradient values at the cost of extra forward computation.
    
    \item Using FlashAttention and implication on model architecture
    \item Precision: FP16/BF16/
    We use mixed precision training using both. However there are caveats regarding both of these two half precision number systems. With BF16, the training was more stable and the loss steadily converged right from the beginning. However, ZeRO-1 optimizer is not supported by default with BF16. To  accommodate ZeRO-1 with BF16 training, we explicitly accumulated gradient in FP32.
    \begin{verbatim}
        "data_types": {
             "grad_accum_dtype": "fp32"
        }
    \end{verbatim}

    Using fp16, the early stages of the training was chaotic, as the loss had very high values. Because BF16 has very high range of values compared to FP16, the formar could support stable loss values.
    
    \item Hand-tuned distribution parameters
    \item DeepHyper tuning results
    \item The recipe for training a Trillion Parameter Model
\end{enumerate}

==> storyline.tex <==
\section*{Storyline}
We start with the background on large LLMs and their usefulness citing the loss scaling laws. Then we emphasise on the fact that a trillion parameter model can really push forward foundational model research, especially after the advent of the 30 Trillion token dataset. Training such a large model on such large dataset requires 120-180 million exaflops and Frontier is the first and only exascale machine. So, we explore the question of how to find an efficient strategy to train such model on Frontier. \textcolor{red}{[Prasanna, Sajal]}

We then explain the Frontier architecture to elaborate its strength (37632 GPUs), capabilities (10 mixed-precision exaflops), and limitations (Communication, lack of AI libraries, etc.). To train a large model on such system requires state of the art distribution techniques, so we survey the state of the art distributed training frameworks such as Megatron-DeepSpeed, FSDP and the types of parallelism they support. \textcolor{red}{[Junqi, Sajal]}

Since Megatron-Deepspeed supports 3D parallelism and have shown numerous success in various large-scale model training, we decide to use this framework and identify the potential component parallelization techniques and the distribution parameters. Since this framework is prepared for NVIDIA hardware, we port this framework through a series of adaptation including hipification and replacing some NVIDIA libraries such as APEX with their ROCM counterpart \textcolor{red}{[Sajal]}. We found that incorporating FlashAttention and FlashAttention 2 significantly boosts the training performance. \textcolor{red}{[Isaac]}

We now explore each of these parallelization techniques and perform experiment on their individual impact on the per GCD throughput. From the first-order understanding of these techniques and parameters, and the experiments, we choose some initial combinations of techniques and associated parameters. \textcolor{red}{[Sajal, Junqi]}

From these initial combinations, we run DeepHyper hyper-parameter tuning to verify our findings and assumptions and readjust our beliefs. Since the search-space is vast and training an individual models is pretty exprensive, we perform this tuning through DeepHyper on a relatively smaller model of size 22B/175B. From the previous step and this step we finalize our training strategies and devise a final recipe for training a Trillion parameter model. \textcolor{red}{[Sajal, Romain]}

In the next section, we put the recipe into test to train three models of size 22B, 175B, and 1T and we achieve 76\%, 72\%, and 66\% of theoretical FLOPs per GCD. We perform some analysis by collecting traces and hardware counter to show why certain strategies work. We demonstrate hardware flops, compute-communication overlap, compute utilization, and roofline for these three models. \textcolor{red}{[Sajal, Xiao]}

A final question remains, how can we train our models using the entire Frontier since it poses a problem of using a really large batch-size. If we assign one sample per GCD, to utilize the full Frontier, we will need (9,408 * 4 * 2) 75264 sequences per batch, which is 155 million tokens. We need to make trade-offs between using the part of the Frontier and achieved throughput per GCD. \textcolor{red}{[Sajal, Junqi]}
